Estimating Unknown Population Sizes Using the Hypergeometric Distribution

The multivariate hypergeometric distribution describes sampling without replacement from a discrete population of elements divided into multiple categories. Addressing a gap in the literature, we tackle the challenge of estimating discrete distributions when both the total population size and the sizes of its constituent categories are unknown. Here, we propose a novel solution using the hypergeometric likelihood to solve this estimation challenge, even in the presence of severe under-sampling. We develop our approach to account for a data generating process where the ground-truth is a mixture of distributions conditional on a continuous latent variable, such as with collaborative filtering, using the variational autoencoder framework. Empirical data simulation demonstrates that our method outperforms other likelihood functions used to model count data, both in terms of accuracy of population size estimate and in its ability to learn an informative latent space. We demonstrate our method's versatility through applications in NLP, by inferring and estimating the complexity of latent vocabularies in text excerpts, and in biology, by accurately recovering the true number of gene transcripts from sparse single-cell genomics data.

==> sim_results_table_full.tex <==
\begin{table*}
\caption{Representative results comparing the hypergeometric (HG), multinomial (MN) and Poisson (P) likelihood estimates on simulated datasets (additional results in Appendix \ref{appendix:extra_results}). Ground-truth distributions are uniformly under-sampled by $20-60\%$. Metrics are adjusted Rand index (ARI), median percentage error (MPE), and mean absolute error (MAE), averaged over 5 simulation random seeds.}
\label{table:results}
\vskip 0.1in
\begin{center}
\begin{scriptsize}
\begin{sc}
% \begin{tabular}{l||m{4em}|m{4em}|m{4em}||m{4em}|m{4em}||m{4em}|m{4em}|}
\begin{tabular}{l||c|c|c||c|c||c|c}
 & \multicolumn{3}{c||}{ARI} & \multicolumn{2}{c||}{MPE} & \multicolumn{2}{c}{MAE} \\
 & HG (ours) & MN & P & HG (ours) & P & HG (ours) & P \\
\hline
% simulation 240125_184331
\makecell{3 distributions (2 unique), $10^3$ categories,\\$10^3$ obs/distribution, $10^4$ ground-truth total} & 
\makecell{$1.00$\\$\pm 0.01$} & \makecell{$0.45$\\$\pm 0.01$} & \makecell{$0.45$\\$\pm 0.15$} & 
\makecell{$2.8$\\$\pm 0.3\%$} & \makecell{$26.1$\\$\pm 0.1\%$} & 
\makecell{$416$\\$\pm 49$} & \makecell{$3471$\\$\pm 2$} \\
\hline
% simulation 240125_204750
\makecell{3 distributions (2 unique), $10^4$ categories,\\$10^4$ obs/distribution, $10^4$ ground-truth total} & 
\makecell{$1.00$\\$\pm 0.01$} & \makecell{$0.45$\\$\pm 0.01$} & \makecell{$0.50$\\$\pm 0.01$} & 
\makecell{$3.9$\\$\pm 0.9\%$} & \makecell{$23.3$\\$\pm 0.8\%$} & 
\makecell{$573$\\$\pm 152$} & \makecell{$3744$\\$\pm 23$} \\
\hline
% simulation 240129_215227
\makecell{10 distributions (9 unique), $10^3$ categories,\\$10^5$ obs/distribution, $10^5$ ground-truth total} & 
\makecell{$0.99$\\$\pm 0.01$} & \makecell{$0.89$\\$\pm 0.01$} & \makecell{$0.87$\\$\pm 0.01$} & 
\makecell{$1.6$\\$\pm 0.1\%$} & \makecell{$6.5$\\$\pm 0.1\%$} & 
\makecell{$225$\\$\pm 6$} & \makecell{$7309$\\$\pm 43$} \\
\hline
% simulation 240129_215230
\makecell{10 distributions, $10^1$ categories,\\$10^3$ obs/distribution, $10^3$ ground-truth total} & 
\makecell{$1.00$\\$\pm 0.01$} & \makecell{$1.00$\\$\pm 0.01$} & \makecell{$0.978$\\$\pm 0.023$} & 
\makecell{$2.5$\\$\pm 0.2\%$} & \makecell{$64$\\$\pm 1\%$} & 
\makecell{$27$\\$\pm 3$} & \makecell{$6.2$\\$\pm 0.1$} \\
\hline
% simulation 240129_220142
\makecell{100 distributions, $10^3$ categories,\\$10^4$ obs/distribution, $10^4$ ground-truth total} & 
\makecell{$0.97$\\$\pm 0.01$} & \makecell{$0.10$\\$\pm 0.04$} & \makecell{$0.98$\\$\pm 0.01$} & 
\makecell{$0.8$\\$\pm 0.1\%$} & \makecell{$0.7$\\$\pm 0.1\%$} & 
\makecell{$99$\\$\pm 11$} & \makecell{$65$\\$\pm 1$} \\
\hline
% simulation 240125_204909
\makecell{3 distributions (2 unique), $10^3$ categories,\\$10^3$ obs/distribution, $10^4$ ground-truth total} & 
\makecell{$0.89$\\$\pm 0.18$} & \makecell{$0.50$\\$\pm 0.01$} & \makecell{$0.50$\\$\pm 0.01$} & 
\makecell{$6.6$\\$\pm 1.2\%$} & \makecell{$23.0$\\$\pm 0.2\%$} & 
\makecell{$1438$\\$\pm 101$} & \makecell{$3772$\\$\pm 17$} \\
\hline
% simulation 240125_204947
\makecell{10 distributions, $10^3$ categories,\\$10^3$ obs/distribution, $10^4$ ground-truth total} & 
\makecell{$1.00$\\$\pm 0.01$} & \makecell{$1.00$\\$\pm 0.01$} & \makecell{$0.72$\\$\pm 0.11$} & 
\makecell{$4.8$\\$\pm 1.2\%$} & \makecell{$10.3$\\$\pm 0.1\%$} & 
\makecell{$485$\\$\pm 119$} & \makecell{$943$\\$\pm 13$} \\
\hline
% simulation 240125_220806
\makecell{10 distributions, $10^3$ categories,\\$10^3$ obs/distribution, $10^5$ ground-truth total} & 
\makecell{$1.00$\\$\pm 0.01$} & \makecell{$1.00$\\$\pm 0.01$} & \makecell{$0.51$\\$\pm 0.11$} & 
\makecell{$9.0$\\$\pm 5.5\%$} & \makecell{$10.3$\\$\pm 0.1\%$} & 
\makecell{$8767$\\$\pm 5331$} & \makecell{$9538$\\$\pm 86$} \\
\hline
% simulation 240129_215527
\makecell{10 distributions, 10 categories,\\$10^5$ obs/distribution, $10^3$ ground-truth total} & 
\makecell{$1.00$\\$\pm 0.01$} & \makecell{$1.00$\\$\pm 0.01$} & \makecell{$0.78$\\$\pm 0.01$} & 
\makecell{$5.2$\\$\pm 1.5\%$} & \makecell{$6.3$\\$\pm 0.1\%$} & 
\makecell{$52$\\$\pm 15$} & \makecell{$63$\\$\pm 1$} \\
\hline
% simulation 240129_214255
\makecell{10 distributions, 100 categories,\\$10^4$ obs/distribution, $10^4$ ground-truth total} & 
\makecell{$1.00$\\$\pm 0.01$} & \makecell{$1.00$\\$\pm 0.01$} & \makecell{$0.89$\\$\pm 0.01$} & 
\makecell{$4.8$\\$\pm 0.1\%$} & \makecell{$6.3$\\$\pm 0.1\%$} & 
\makecell{$481$\\$\pm 12$} & \makecell{$633$\\$\pm 1$} \\
\hline
% simulation 240129_215229
\makecell{10 distributions (9 unique), 10 categories,\\$10^4$ obs/distribution, $10^3$ ground-truth total} & 
\makecell{$0.89$\\$\pm 0.01$} & \makecell{$0.89$\\$\pm 0.01$} & \makecell{$0.89$\\$\pm 0.01$} & 
\makecell{$3.5$\\$\pm 0.1\%$} & \makecell{$6.5$\\$\pm 0.1\%$} & 
\makecell{$48$\\$\pm 12$} & \makecell{$73$\\$\pm 1$} \\
\hline

\end{tabular}
\end{sc}
\end{scriptsize}
\end{center}
\vskip -0.1in
\end{table*}
